Deep Synoptic Monte Carlo Planning in Reconnaissance Blind Chess

This paper introduces deep synoptic Monte Carlo planning (DSMCP) for large imperfect information games. The algorithm constructs a belief state with an unweighted particle filter and plans via playouts that start at samples drawn from the belief state. The algorithm accounts for uncertainty by performing inference on "synopses," a novel stochastic abstraction of information states. DSMCP is the basis of the program Penumbra, which won the official 2020 reconnaissance blind chess competition versus 33 other programs. This paper also evaluates algorithm variants that incorporate caution, paranoia, and a novel bandit algorithm. Furthermore, it audits the synopsis features used in Penumbra with per-bit saliency statistics.

==> checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{The synopsis abstraction makes DSMCP tractable for large games, and the experiments show that the stochastic bandit algorithm contributes significantly to the algorithm's performance.}
  \item Did you describe the limitations of your work?
    \answerYes{The paper is upfront that DSMCP does not explicitly seek a Nash equilibrium.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{The broader impact section mentions how algorithms that are capable of planning in large domains involving uncertainty (such as the real world) could have harmful applications.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{The main paper does not contain theoretical results, though the appendix may include statements about of the asymptotic behavior of the stochastic bandit algorithm and of DSMCP.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{The main paper does not contain theoretical results, though the appendix may include of proofs the theoretical statements in it.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{While it is not released yet, the games produced in the experiments will be shared and the algorithms will be contributed to an open source suite of algorithms.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNo{For example, the random seeds and precise makeup of the \focustop{} dataset are not provided, but the paper does make a best-effort to provide as many details as possible which are likely to be sufficient to reproduce the results.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{The experiments contains 95\% confidence intervals for the provided Elo ratings.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Section~\ref{sec:training-procedure} mentions the four RTX 2080 Ti GPUs used.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Section~\ref{sec:reconnaissance-blind-chess} cites the creators of reconnaissance blind chess, and Section~\ref{sec:experiments} cites the authors of the baseline programs used in the experiments.}
  \item Did you mention the license of the assets?
    \answerNo{It looks like Johns Hopkins University has not provided an explicit license for the board game or the games played on the website.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Additional assets will be provided in the supplementary material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{The paper does not explicitly discuss receiving consent for participating in the RBC contest or training on RBC games, which seems okay.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{Whether or not a person or program can be identified by what moves are chosen in a game of RBC is an interesting research question, but it is tangential and seems acceptable to omit in this paper.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

